Opti-Acoustic Semantic SLAM with Unknown Objects in Underwater Environments

Despite recent advances in semantic Simultaneous Localization and Mapping (SLAM) for terrestrial and aerial applications, underwater semantic SLAM remains an open and largely unaddressed research problem due to the unique sensing modalities and the object classes found underwater. This paper presents an object-based semantic SLAM method for underwater environments that can identify, localize, classify, and map a wide variety of marine objects without a priori knowledge of the object classes present in the scene. The method performs unsupervised object segmentation and object-level feature aggregation, and then uses opti-acoustic sensor fusion for object localization. Probabilistic data association is used to determine observation to landmark correspondences. Given such correspondences, the method then jointly optimizes landmark and vehicle position estimates. Indoor and outdoor underwater datasets with a wide variety of objects and challenging acoustic and lighting conditions are collected for evaluation and made publicly available. Quantitative and qualitative results show the proposed method achieves reduced trajectory error compared to baseline methods, and is able to obtain comparable map accuracy to a baseline closed-set method that requires hand-labeled data of all objects in the scene.

==> figs/cam_sonar_geometry.tex <==
\begin{figure}[h] 
\center
  \includegraphics[width=8cm]{imgs/camera_sonar_geometry.png}
  \caption{}
  \label{fig:cam_sonar_geometry}
\end{figure}  

==> figs/fig_intro2.tex <==
\begin{figure}[h] 
\center
  \includegraphics[width=.99\linewidth]{imgs/intro1.png}
  \caption{intro}
  \label{fig:intro}
\end{figure}  

==> figs/fig_otpi-acoustic.tex <==
\begin{figure}  
    % \vspace{2mm}
    \centering
    \scalebox{0.95}{\input{figs/opti-acoustic_raw}}
    \caption{pipeline}  
    \label{fig:opti-acoustic_temp}
    % \vspace{-4mm}
\end{figure}

==> figs/fig_ping2range_alg2.tex <==
\makeatletter
\newcommand{\algorithmfootnote}[2][\footnotesize]{%
  \let\old@algocf@finish\@algocf@finish% Store algorithm finish macro
  \def\@algocf@finish{\old@algocf@finish% Update finish macro to insert "footnote"
    \leavevmode\rlap{\begin{minipage}{\linewidth}
    #1#2
    \end{minipage}}%
  }%
}
\makeatother
\begin{algorithm}[tb]
  \caption{Find Acoustic Range from Image Bearing}\label{algorithm1}
  \algorithmfootnote{$y_0$ denotes the initial value.}
  \KwIn{this text}
  \KwOut{how to write algorithm with \LaTeX2e }
  initialization\;
  \While{not at end of this document}{
    read current\;
    \eIf{understand}{
      go to next section\;
      current section becomes this one\;
      }{
      $y_0 \leftarrow y$\;
    }
  }
\end{algorithm}


% \caption{Find Acoustic Range from Image Bearing}
% \begin{algorithmic}[1] % Enables line numbering
% \Procedure{Bearing2Range}{$\theta$} % A is the array input
% \State $\theta_{s}^{\text{res}}$ = SONAR\_FOV/NUMBER\_OF\_BEAMS \tab\tab \Comment{Find angular resolution of Sonar}
% \For{beam \textbf{in} beams}
% % \If{ Angle(beam) $\geq \theta - \text{ang\_res}/2$ 
% %     \textbf{and} \\  \tab\tab\tab Angle(beam)$\leq\theta + \text{ang\_res}/2$}
% %     \State $\theta_{s}$ = Angle(beam)
% %     \If{Ping($\theta_{s}$) $\geq$ THRESHOLD}
% %     \State $\text{Range}_{s}$ = Ping($\theta_{s}$)
% \If{ $\theta_{s}$(beam) $\geq \theta - \theta_{s}^{\text{res}}/2$ 
%     \textbf{and} \\  \tab\tab\tab $\theta_{s}$(beam)$\leq\theta + \theta_{s}^{\text{res}}/2$}
%     \If{max(Ping($\theta_{s}$(beam))) $\geq$ $\tau$\footnotemark}
%     \State $\text{Range}_{s}$ = max(Ping($\theta_{s}$(beam)))
%     \State \Return $\text{Range}_{s}$
%     \ElsIf{}
%     \State \Return FALSE
%     \EndIf
% \EndIf
% \EndFor
% \EndProcedure

==> figs/overview_fig.tex <==
\begin{figure*}[ht]
\includegraphics[width=\textwidth, height=5cm]{imgs/0.5504_image_1705883144217558406_image_1705883345652191591.jpg}
\caption{Overview figure placeholder}
\label{fig:overview}
\end{figure*}


==> figs/sonar-range-challenge.tex <==
\begin{figure}[h]
\includegraphics[width=\columnwidth]{imgs/sonar-range-challenge2.png}
\caption{Top left: input image of lobster cage. Top right: Detected object. Bottom: Corresponding sonar frame used for object range estimation. Sonar data can often be noisy and is subject to multi-path effects that make the detection and range extraction of objects challenging. Our method is largely robust to such issues through the use of a probabilistic data association method that takes into account the range uncertainty that is typical with the use of sonar.}
\label{fig:sonar_range_challenge}
\end{figure}


==> figs/sys_diagram.tex <==
\begin{figure}[h] 
\center
  \includegraphics[width=.8\linewidth]{imgs/sys_diagram.png}
  \caption{}
  \label{fig:sys_diagram}
\end{figure}  
